Parallel Implementations for Computing the Minimum Distance of a Random Linear Code on Multicomputers

The minimum distance of a linear code is a key concept in information theory. Therefore, the time required by its computation is very important to many problems in this area. In this paper, we introduce a family of implementations of the Brouwer-Zimmermann algorithm for distributed-memory architectures for computing the minimum distance of a random linear code over F2. Both current commercial and public-domain software only work on either unicore architectures or shared-memory architectures, which are limited in the number of cores/processors employed in the computation. Our implementations focus on distributed-memory architectures, thus being able to employ hundreds or even thousands of cores in the computation of the minimum distance. Our experimental results show that our implementations are much faster, even up to several orders of magnitude, than current implementations widely used nowadays.

==> old/crc_tex_toms_rev2/0_Abstract.tex <==

The minimum distance of an error-correcting code is an important concept in information theory.
Hence, computing the minimum distance of a code 
with a minimum computational cost is crucial to many problems in this area.
%
In this paper, we present and assess
a family of implementations
of both the brute-force algorithm and the Brouwer-Zimmermann algorithm
for computing 
the minimum distance of a random linear code over $\mathbb{F}_{2}$
that are faster than current implementations, 
both in the commercial and public domain.
In addition to the basic sequential implementations,
we present parallel and vectorized implementations that
produce high performances on modern architectures.
%
The attained performance results show the benefits of the
developed optimized algorithms, which obtain remarkable 
improvements compared with state-of-the-art implementations widely
used nowadays.



==> old/crc_tex_toms_rev2/1_Introduction.tex <==
% =============================================================================
\section{Introduction}
% =============================================================================

Coding theory  studies methods for detecting and correcting errors after sending digital information  through an unreliable communication channel.
Nowadays, it is a well-established discipline \cite{MacWilliams} and it is widely used in a number of fields, such as 
data compression~\cite{Ancheta,Liveris}, 
code-based cryptography~\cite{Nie,McEl,Wang16},
network coding~\cite{Li,Zhang06},
secret sharing~\cite{Shamir,Olav,Karnin83,McEliece81},
list decoding~\cite{Guruswami11},
mobile broadcasting communications~\cite{Nazir11} and
recovery of data stored in networks~\cite{Sipos15,Lin07}, among others.
The most studied codes are linear codes, i.e., vector subspaces of
dimension $k$ within a vector space of dimension $n$ over a finite field, 
and the minimum Hamming distance is the most common way of quantifing  how many errors can be detected or corrected. It is well known that if the minimum Hamming distance of a linear code is $d$, then $d-1$ errors can be detected, and
$\lfloor (d-1)/2 \rfloor$ errors can be corrected.
Therefore,  knowledge of the minimum distance 
of a linear code is essential to determining 
how well it will perform.
Coding theory is an active research area because the discovery of better codes
with larger distances can improve the recovery and fault-tolerance
of transmission channels.

Computing the minimum distance of a linear code is an important
task but also a complex one. 
Actually, several authors~\cite{NPHard,Vardy} 
proved that it is an NP-hard problem, 
and the corresponding decision problem is NP-complete.
%%%% The computation of the minimum distance of a random linear code is 
%%%% an NP-hard problem~\cite{NPHard,Vardy}.
Whereas this problem is unfeasible for large dimensions,
it can be efficiently solved in a reasonable time 
for small values of $k$ and $n$.
In modern computers,
feasible values for $k$ are usually smaller than one hundred, 
and feasible values for $n$ are usually smaller than a few hundred.

Since larger minimum distances allow one 
to detect and recover a larger number of errors,
the interest in computing and designing linear codes 
with larger minimum distances is very high.
There are some web pages~\cite{cota}
that store the best minimum distance 
known to date for a large range of dimensions $k$ and lengths $n$.

The fastest general algorithm 
for computing the minimum distance of a random linear code
is the so-called Brouwer-Zimmermann algorithm~\cite{Zim},
which is described in detail in~\cite{Grassl}.
This algorithm has been implemented 
in \magma{}~\cite{Magma} over any finite field,
and in GAP (package \guava{})~\cite{GAP,Guava}
over the  fields $\mathbb{F}_2$ and $\mathbb{F}_3$.

In this paper, we present 
a family of new implementations 
of both the brute-force algorithm and the Brouwer-Zimmermann algorithm
for computing the minimum distance of random linear codes
over $\mathbb{F}_2$. 
The key advantage of the new implementations is twofold:
they perform fewer row additions than the traditional ones, and
they increase the ratio of row additions to row accesses.
%
Our new implementations are faster than current ones,
both commercial and public-domain, when using only one CPU core.
Also, our new implementations 
can take advantage of modern architectures with multiple cores, and  produce  higher performances than available implementations on multicore architectures.
Moreover, our new implementations can take advantage of 
SIMD (single-instruction, multiple-data)
instructions available in old and modern processors 
to attain even higher performances.
%
Armed with all these improvements, the time required to compute the minimum
distance of a linear code can be drastically reduced
in comparison with current implementations. Although our implementations only work for $\mathbb{F}_2$, our ideas can be applied to other finite fields.
%
%We believe that the scientific community can benefit from our work
%because the minimum distance of random linear codes can be computed
%much more quickly on serial and multicore architectures
%by using our new algorithms and implementations.

The rest of the paper is structured as follows.
Section~\ref{sec:background} introduces the mathematical background
of the problem and the classical approaches typically employed to solve it,
together with their computational challenges.
Section~\ref{sec:new_algorithms} proposes our family of new algorithms 
for tackling this problem, showing them in an incremental fashion 
as we introduce several improvements 
that reduce their computational complexity
and thus improve performance on modern computing architectures.
Section~\ref{sec:implementation_and_optimization} reports implementation
details to adapt the new algorithms to modern parallel
computing architectures.
Section~\ref{sec:performance_analysis} analyzes the performance 
attained by our new algorithms on different modern architectures, 
comparing them with state-of-the-art alternative implementations.
In Section~\ref{sec:new_codes}, we leverage our new algorithms 
to generate some new linear codes better than any previously known for $n=232-236$ and $k=51-52$ .
Finally, Section~\ref{sec:conclusions} closes the paper with some
concluding remarks.




==> old/crc_tex_toms_rev2/2_Background.tex <==
% =============================================================================
\section{Background}
\label{sec:background}
% =============================================================================

Let $q=p^r$ be a prime power, 
we denote by $\mathbb{F}_q$ the finite field with $q$ elements. 
By a linear code over $\mathbb{F}_q$, 
say $C$, we mean a $k$-dimensional $\mathbb{F}_q$ vector subspace 
of $\mathbb{F}_q^n$, $n > k$, i.e., 
it is the image of an injective map 
$i:\mathbb{F}_q^k\hookrightarrow \mathbb{F}_q^n$.
As any linear map, $i$ is given by a $k\times n$ matrix $G$ whose rows are
a basis of $C$. In coding theory, $G$ is called a generator matrix.
Since it has rank $k$, 
it can be written, after permutation of columns and elementary row  operations,
in the systematic form $\Gamma=(I_k\mid A)$, 
where $A$ is a $k\times (n-k)$ matrix,
and $I_k$ is the identity matrix of dimension $k$.

Therefore, if we want to encode a sequence of $k$ elements in $\mathbb{F}_q$, 
say $(c_1,\ldots,c_k)$, 
we simply multiply 
$(c_1,\ldots,c_k)(I_k\mid A) = (c_1,\ldots,c_k,c_{k+1},\ldots,c_n)$.
Thus, we introduce $n-k$ redundancy elements in $\mathbb{F}_q$, 
which will eventually be useful to correct the information 
in case it has been corrupted.
A linear code C as above contains $q^k$ codewords. 
When a codeword 
$(c_1,\ldots,c_n)$
is sent through a noisy channel,
an error $e=(e_1,\ldots,e_n)$ might appear in the received word
$r=(c_1,\ldots,c_n)+(e_1,\ldots,e_n)$.
The method to find out which codeword was sent when $r$ is received
is to replace $r$ with the nearest codeword.
In order to do so, we need a metric.
Given two vectors in $\mathbb{F}_q^n$,
say $a=(a_1,\ldots,a_n)$ and $b=(b_1,\ldots,b_n)$, 
we define the Hamming distance of $a$ and $b$ 
as the number of positions where they differ, i.e.,

\[
  \dd( a, b )=\#\{ i \mid a_i \ne b_i \}.
\]

Hence, the minimum distance of a linear code is defined as follows:
\[
  \dd(C) = \min\{ \dd( a, b ) \mid a, b \in C \}.
\]

It is quite useful to define the weight of a vector
$a=(a_1,\ldots,a_n)\in \mathbb{F}_q^n$  to be the number of non-zero
positions, i.e.,
\[
  \wt( a ) = \#\{ i \mid a_i \ne 0 \} = \dd( a, 0 )
  \;\; \textrm{and then } \;\;
  \dd( a, b ) = \wt( b - a ).
\]

So, the minimum weight of a linear code is:

\[
  \wt( C ) = \min\{ \wt( a ) \mid a \in C \}.
\]

Since $C$ is a linear subspace, it is easy to prove that $\wt(C)=\dd(C)$.  
%%%% but computing the weight requires $q^k$ measurements
%%%% whereas computing the minimum distance requires $\binom{q^k}{2}$.
Note that straightforwardly computing the minimum weight from the definition
would use $O( n q^k )$ field operations,
whereas computing the minimum distance would use $O( n \binom{q^k}{2} )$.

It is customary to say that a linear code $C$ over $\mathbb{F}_q$ has parameters $[n,k,d]_q$ 
if it has length $n$, dimension $k$, and minimum distance $d$. From now onwards, 
we will use $\dd$ instead of $\dd(C)$ when $C$ is known.
With it, we represent either the minimum distance or the minimum weight.
This number is essential because, as mentioned in the introduction, $\lfloor (d-1)/2 \rfloor$ is
the number of errors that can be corrected using the nearest codeword method.
If the received word is equidistant to two or more codewords,
then it cannot be decided which one of them was the one sent.
But as far as $\wt(e)\le \lfloor (d-1)/2 \rfloor$, 
the nearest codeword to the received one is unique.

From now on we will only consider codes over $\mathbb{F}_2$.

The simplest algorithm 
for computing the minimum distance of a random linear code
is a trivial brute-force algorithm, where
all combinations of the $k$ rows taken from 1 up to $k$ rows at a time
are considered.
In fact, it is not necessary to follow any specific order 
whenever all the combinations are processed;
for each generated combination, the corresponding rows are added,
and then the overall minimum weight is updated.
This algorithmic approach is outlined in Algorithm~\ref{alg:brute-force}.

\begin{algorithm}[ht!]
  \caption{\ensuremath{\mbox{\sc Brute-force algorithm}}}
  \label{alg:brute-force}
  \begin{algorithmic}[1]
    \REQUIRE A generator matrix $G$ of the linear code $C$ with
             parameters $[n,k,d]$.
    \ENSURE  The minimum weight of $C$, i.e., $d$.
    \medskip
    \STATE \textbf{Beginning of Algorithm}
    \FOR{ $i = 1, 2, \ldots, 2^k - 1$ }
      \STATE $ b = \textrm{convert\_into\_binary\_with\_k\_bits}( i )$;
      \STATE $ c = b \cdot G$;
      \STATE $ d = \min( d, \textrm{weight}( c ) )$;
    \ENDFOR
    \STATE \textbf{End of Algorithm}
  \end{algorithmic}
\end{algorithm}

This brute-force algorithm is simple and easy to implement in exchange 
for an exponential cost as $k$ grows;
in fact, the cost doubles as $k$ increases by one unit.
Hence, cheaper methods have been developed to tackle this problem.

The fastest general algorithm
for computing the minimum distance of a random linear code (to our knowledge) 
is the Brouwer-Zimmermann algorithm~\cite{Zim}, 
which is explained in detail in~\cite{Grassl}.
It is implemented, with some improvements, in \magma{}~\cite{Magma} 
over any finite field.
It is also implemented in GAP (package \guava{})~\cite{GAP} 
over the fields $\mathbb{F}_2$ and $\mathbb{F}_3$.

The main advantage of the Brouwer-Zimmermann is an earlier termination:
it can finish before processing all the combinations of the rows,
thus greatly reducing the overall cost. The method by Brouwer-Zimmermann algorithm is outlined in Algorithm~\ref{alg:BZ},
and it is based on so called information sets.
Given a linear code $C$ with parameters $[n,k,d]$ and a generator matrix $G$,
an information set $S = \{i_1,\ldots,i_k\}\subset \{1,\ldots,n\}$ 
is a subset of $k$ indices such that the corresponding columns of $G$ are 
linearly independent.

The first step is to apply permutations of columns and 
elementary row operations
in order to obtain an initial information set $S_1$ 
and a systematic matrix $\Gamma_1 = ( I_k \mid A_1 )$.

The second step is to find another information set $S_2$ in $A_1$, if possible.
After some permutations and the diagonalization of the leftmost part of $A_1$,
we define the following:
$\Gamma_2=(B_2 \mid I_k \mid A_2)$.
This process is repeated until no more full-rank matrices are found in $A_i$.

Assuming that we have been able to find $m-1$ disjoint information sets
($S_1\cap\cdots\cap S_{m-1}=\emptyset$), 
then we get $m-1$ different matrices $\Gamma_j = ( B_j \mid I_k \mid A_j )$.
%
Lisonek et al.~\cite{Lisonek15}
described an interesting method that uses matroids
to find good disjoint informations sets.
%
In this case,
the rank $k_{m-1}$ of $A_{m-1}$ is strictly less than $k$.
Then, after applying column permutations and row operations,
the following is obtained:
\[
  \Gamma_m = \left( 
              \begin{array}{c|c|c}
                B_m 
                & 
                \begin{matrix}
                  I_{k_{m-1}} \\     
                  0           
                \end{matrix}
                &
                \begin{matrix}
                  A_m \\     
                  0           
                \end{matrix} \\
              \end{array}
            \right).
\]

The total number of $\Gamma$ matrices is $m$.
The first $m-1$ $\Gamma$ matrices have full rank $k$
in the columns corresponding to the informations sets.
In contrast,
the last $\Gamma$ matrix has rank $k_{m-1} < k$
in the remaining columns (those not in the information sets).

The basic idea in the Brouwer-Zimmermann algorithm
is to consider an upper bound $U$ and a lower bound $L$ of the minimum distance of the code.
The upper bound $U$ is initialized to $n-k+1$
since the Singleton's bound states 
that $d \leq n - k + 1$~\cite[p.~33]{MacWilliams}.
The lower bound $L$ is initialized to $1$.
Then, both bounds are updated after enumerating codewords,
and it is checked whether $L \ge U$; 
if so, the process can stop and the minimum weight is $U$.

The codewords are enumerated as follows: 
First, all the combinations of the $k$ rows taken one at a time are considered.
That is, all the linear combinations $c \cdot \Gamma_j$ for $j=1,\ldots,m$,
where $c=(c_1,\ldots,c_k)$ and $\wt(c)=1$
(since we are over $\mathbb{F}_2$, it means that all $c_i$ are zero but one).
After computing every linear combination, 
the upper bound is updated in the following way:
If the new weight is smaller than the upper bound $U$, 
then $U$ is set to the new weight (line 7 in Algorithm~\ref{alg:BZ}).
When all $\Gamma_j$ matrices have been processed
(in this step the combinations still contain only one row),
the lower bound $L$ is updated in the following way:
The lower bound $L$ is increased by one unit 
for every disjoint information set
because $c \cdot \Gamma_j$ has $g$ ones 
in the positions $(j-1)k+1, \ldots, jk$,
so we can guarantee that $\wt( c \cdot \Gamma_j ) \geq g$.
Hence, in every consecutive step ($g \rightarrow g+1$) 
the weight of the enumerated codeworks increases at least by one.
Moreover, 
note that the matrix $\Gamma_m$ has rank $k_{m-1}$ 
in the columns from $(m-1)k+1,\ldots,n$,
so we have to check whether the weight is increased by one.
It will contribute with one unit whenever $k_{m-1} - k + g + 1 > 0$.
%%%% There are at least $m-1$ disjoint information sets,
%%%% and as many as one that is not full rank.
%%%% However, all information sets, both full rank and rank defficient,
%%%% must be processed in line 5 in Algorithm~\ref{alg:BZ}.
Line 9 in Algorithm~\ref{alg:BZ} performs such updating.

Then, the above process is repeated for the combinations of the $k$ rows 
taken two rows at a time. And so on.
This process is repeated
until the lower bound $L$ is greater than or equal to the upper bound $U$.

The ability to terminate earlier is very important 
because it can accelerate the overall procedure.
One important drawback is to have to process several $\Gamma$ matrices.
See~\cite{Grassl} for more details.

%%%% Moreover, after processing all those linear combinations
%%%% $c\cdot\Gamma_j$ for $j=1,\ldots,m$,
%%%% the lower bound is increased by $m-1$ units 
%%%% (actually one after each $\Gamma_j$) for the disjoint information sets 
%%%% and a different quantity if the information sets are not disjoints
%%%% (closed formula). 
%%%% See \cite{Grassl} for more details.
%%%% Now the same procedure is repeated for linear combinations 
%%%% $c\cdot\Gamma_j$ for $j=1,\ldots,m$ and $\wt(c)=2$. 
%%%% Then, the same is done for $\wt(c)=3$, 
%%%% and so on until $L\ge U$ is obtained.

\begin{algorithm}[ht!]
  \caption{\ensuremath{\mbox{\sc Minimum weight algorithm 
                                 for a linear code $C$}}}
  \label{alg:BZ}
  \begin{algorithmic}[1]
    \REQUIRE A generator matrix $G$ of the linear code $C$ with 
             parameters $[n,k,d]$.
    \ENSURE The minimum weight of $C$, i.e., $d$.
    \medskip
    \STATE \textbf{Beginning of Algorithm}
    \STATE [ $\Gamma_j$ ] = Compute\_gamma\_matrices( G );
    \STATE $L = 1$; $U = n-k+1$;
    \STATE $g = 1$;
    \WHILE{ $g \le k$ and $L < U$  }
      \FOR{$ j = 1,\ldots, m $}
         \STATE $U = \min\{ U, \min\{\wt( c\Gamma_j ) : 
                 c \in \mathbb{F}_2^k \mid \wt(c)=g\}\}$ ;
      \ENDFOR
      \STATE $L = (m-1)(g+1)+\max\{0,g+1-k+k_{m-1}\}$ ;
      \STATE $g = g+1$;
    \ENDWHILE
    \STATE $d$ = $U$;
    \STATE \textbf{End of Algorithm}

    \medskip

    \STATE \textbf{Function} Compute\_gamma\_matrices( G ) \textbf{is:}
    \STATE // Return G after diagonalizing leading block (1:k,1:k),
    \STATE // then return G after diagonalizing second block (1:k, k+1:2k), 
              and so on.
    \STATE \textbf{End of Function}
  \end{algorithmic}
\end{algorithm}

It is clear from line 9 in Algorithm~\ref{alg:BZ}
that the lower bound increases linearly in steps of $m-1$ units.
So, the more disjoint information sets there are,
the more quickly the lower bound increases.
Hence, the algorithm will finish earlier if $m$ is large and, in consequence,
the final $g$ will be smaller.
Recall that $g$ is the number of rows in a combination.

Notice that the number of linear combinations of weight $\leq g$ is
$N = \sum_{j=1}^g \binom{k}{j}$.
For small values of $g$ we have that $N<\binom{k}{g+1}$, 
so increasing by one the value of $g$
will require a cost as large as 
the addition of the cost of all the previous values of $g$.
We actually have the following result.

\begin{lemma}
Using the previous notation, if $g\le \frac{k}{3}$, then
\[
  \sum_{j=1}^{g-1} \binom{k}{j} < \binom{k}{g}.
\]
\end{lemma}
\begin{proof}
First of all we have that $\binom{k}{g}=\frac{k-g+1}{g}\binom{k}{g-1}$.
Since $g\le \frac{k}{3}$ it holds that
$\binom{k}{g}>2\binom{k}{g-1}=\binom{k}{g-1}+\binom{k}{g-1}>\binom{k}{g-1}+2\binom{k}{g-2}>\cdots
>\sum_{j=1}^{g-1} \binom{k}{j}$, which concludes the proof.
\end{proof}

It is quite clear that the most computationally intensive part of this method
is the computation of those linear combinations of the $g$ rows
of every matrix $\Gamma_j$,
since 
the cost of generating all linear combinations is combinatorial,
whereas
the cost of the diagonalization to obtain the $\Gamma_j$ matrices is $O(n^3)$.
In the following, we will focus on the efficient computation of 
the linear combinations to speed up this algorithm.




==> old/crc_tex_toms_rev2/3_Algorithms.tex <==
% =============================================================================
\section{New algorithms}
\label{sec:new_algorithms}
% =============================================================================

As the most time-consuming part is the generation of linear combinations,
we are going to focus on that component
of both the brute-force algorithm and the Brouwer-Zimmermann algorithm.

%%%% Its basic goal is simple:
%%%% For every $\Gamma$ matrix, the additions of all the combinations of
%%%% its rows must be computed,
%%%% and then the minimum of the weights of those additions
%%%% must be computed.
%%%% The combinations of the $k$ rows of the $\Gamma$ matrices
%%%% are generated
%%%% first taking one row at a time,
%%%% then taking two rows at a time,
%%%% then taking three rows at a time,
%%%% etc.
%%%% The minimum of those weights must be computed,
%%%% and when the minimum value ($L$) is equal to or larger than 
%%%% the upper value ($U$),
%%%% this iterative process finishes.

We have designed several algorithms to perform this task.
The basic goals of the new algorithms for obtaining better performances
are the following:
\begin{enumerate}
\item  Reduction of the number of row addition operations.
\item  Reduction of the number of row access operations.
\item  Increase of the ratio of the number of row addition operations to
       the number of row access operations.
\item  Use of cache-friendly data access patterns.
\item  Parallelization of the serial codes 
       so that all the cores in the system are used.
\item  Vectorization of the serial and parallel codes
       to exploit the SIMD/vector machine instructions and hardware units.
\end{enumerate}

Unlike the previous algorithm,
the next algorithmic descriptions do not show the termination condition
nor the updates of $L$ and $U$ 
so that the notation is not complicated unnecesarily.

In the following, we describe in detail the algorithms implemented in this work
by first introducing the optimization of the brute-force algorithm 
(Subsection~\ref{alg:brute_desc}) 
and then the optimizations applied to the Brouwer-Zimmermann algorithm.
These optimizations are the following:
a basic algorithm (Subsection~\ref{alg:basic_desc}),
an optimized algorithm (Subsection~\ref{alg:optimized_desc}),
the stack-based algorithm (Subsection~\ref{alg:stack-based_desc}),
the algorithm with saved additions (Subsection~\ref{alg:stack-based-additions_desc}), and
the algorithm with saved additions and unrollings (Subsection~\ref{alg:stack-based-additions-unroll_desc}).
In all algorithms, we assume that vector and matrix indices start at zero.


% -----------------------------------------------------------------------------
\subsection{Brute-force algorithm with Gray code based enumeration\label{alg:brute_desc}}
% -----------------------------------------------------------------------------

The brute-force algorithm presented above
performs a lot of additions for every combination (iteration of the $i$ loop):
If there is a one in the $j$-th position of the binary code,
then the $j$-th row of $G$ must be added.
Since the additions of rows is one of the most time-consuming parts
of this algorithm, it is very important to reduce this number.

This number of additions can be reduced by using a Gray code based enumeration
because in this enumeration there is only one difference 
between the current element in the sequence and the next one.
By using this enumeration,
the current addition of rows can be reused 
to generate the next addition of rows,
thus saving many of them.
This new algorithm is outlined in Algorithm~\ref{alg:gray-code-brute-force}.

\begin{algorithm}[ht!]
  \caption{\ensuremath{\mbox{\sc Brute-force algorithm 
                                 with Gray code based enumeration}}}
  \label{alg:gray-code-brute-force}
  \begin{algorithmic}[1]
    \REQUIRE A generator matrix $G$ of the linear code $C$ with
             parameters $[n,k,d]$.
    \ENSURE  The minimum weight of $C$, i.e., $d$.
    \medskip
    \STATE  \textbf{Beginning of Algorithm}
    \FOR{ $i = 1, 2, \ldots, 2^k - 1$ }
      \STATE  $ b = \textrm{convert\_into\_gray}( i )$;
      \IF{ ( $i == 1$ )}
        \STATE  addition = $b \cdot G$ ;
      \ELSE
        \STATE  j = Find\_the\_difference\_between( b, previous\_code );
        \STATE  addition = addition + $j$-th row of $G$;
      \ENDIF
      \STATE  previous\_code = $b$;
      \STATE  $ d = \min( d, \textrm{weight}( \textrm{addition} ) )$;
    \ENDFOR
    \STATE \textbf{End of Algorithm}
  \end{algorithmic}
\end{algorithm}

Notice that this algorithm
performs just one addition of rows in every iteration of the $i$ loop.
Therefore, the total number of additions is $2^k - 1$.
The main advantage of this algorithm is the reduced number of row additions.
The main drawback of this algorithm is that 
$2^k - 1$ combinations must always be processed
because there is no early termination.


Next, we describe several algorithms based on the Brouwer-Zimmermann approach.
Their main advantage is that they can finish much earlier without
evaluating all the combinations of the $k$ rows.
Their main drawback is that they must process several $\Gamma$ matrices
instead of a single $G$ matrix.


% -----------------------------------------------------------------------------
\subsection{Basic algorithm\label{alg:basic_desc}}
% -----------------------------------------------------------------------------

The most basic algorithm is straightforward:
If a $\Gamma$ matrix has $k$ rows,
all the combinations of the $k$ rows taken
with an increasing number of rows are generated.
For every generated combination, the corresponding rows are added,
and the overall minimum weight is updated.
The basic algorithm is outlined in Algorithm~\ref{alg:basic}.
Note that in this algorithm and the following ones
a combination is represented as a sequence of row indices.

\begin{algorithm}[ht!]
  \caption{\ensuremath{\mbox{\sc Basic algorithm}}}
  \label{alg:basic}
  \begin{algorithmic}[1]
    \REQUIRE A generator matrix $G$ of the linear code $C$ with
             parameters $[n,k,d]$.
    \ENSURE  The minimum weight of $C$, i.e., $d$.
    \medskip
    \STATE \textbf{Beginning of Algorithm}
    \STATE [ $\Gamma_j$ ] = Compute\_gamma\_matrices( G );
    \FOR{ $g = 1, 2, \ldots$ }
      \FOR{ every $\Gamma$ matrix ($k \times n$) of $G$ }
        \STATE // Process all combinations of the $k$ rows of $\Gamma$ 
                  taken $g$ at a time:
        \STATE ( done, c ) = Get\_first\_combination();
        \WHILE{( ! done )}
          \STATE Process\_combination( c, $\Gamma$ );
          \STATE ( done, c ) = Get\_next\_combination( c );
        \ENDWHILE
      \ENDFOR
    \ENDFOR
    \STATE \textbf{End of Algorithm}

    \medskip

    \STATE \textbf{Function} Get\_first\_combination() \textbf{is:}
    \STATE Return ( true, $(0,1,2,\ldots,g-1)$ )
    \STATE \textbf{End of Function}

    \medskip

    \STATE \textbf{Function} Get\_next\_combination( c ) \textbf{is:}
    \STATE done = Is\_this\_the\_last\_combination( c );
    \STATE c = Compute\_the\_next\_combination\_to\_be\_processed\_after( c );
    \STATE Return ( done, c )
    \STATE \textbf{End of Function}

    \medskip

    \STATE \textbf{Function} Process\_combination( c, $\Gamma$ ) \textbf{is:}
    \STATE // Compute the weight of the addition of the 
              rows of $\Gamma$ with indices in c.
    \STATE // Update the lower and upper bounds, if needed.
    \STATE \textbf{End of Function}
  \end{algorithmic}
\end{algorithm}


The first step of this algorithm computes the $\Gamma$ matrices
out of the generator matrix $G$.
As has already been mentioned,
this process is usually very fast in comparison to the rest of the algorithm.
As it is so cheap,
this algorithm (and the next ones)
compute the $\Gamma$ matrices of several random permutations 
of the original generator $G$ 
in order to find one permutation 
with the largest number of full-rank $\Gamma$ matrices and 
the largest rank in the last $\Gamma$ matrix.
The larger those valules, 
the sooner the following iterative process will finish.
In our implementations we have computed 10 permutations,
but this parameter can be easily set up before every computation.

The main part of the algorithm 
(the computation of all the combinations of the rows of a given $\Gamma$ matrix
taken $g$ at a time)
could have been implemented recursively,
but this type of implementation is usually slow 
if the computational cost inside every call is small
in comparison to the call overhead.
Hence, to avoid this overhead
we used an iterative implementation instead.

%%%% Each combination $c$ will contain $g$ indices of the rows of 
%%%% the current $\Gamma$ matrix being processed.
The order in which these combinations are generated is not important
in this algorithm.
However, in our implementation the lexicographical order was used
since it is very cache-friendly 
due to the fact that it accesses the rows in a serial way.

This algorithm stops as soon as the overall minimum weight 
after processing a $\Gamma$ matrix
is equal to or larger than the upper value.

Notice that this algorithm
performs $g-1$ additions of rows for every $g$ rows brought 
from the main memory.
Hence, as the ratio of row additions to row accesses is so low,
it might not be able to extract all the computing power
from the processors, and the speed of the main memory
could ultimately define the overall performance of the implementation.
If we wish to obtain better performances, one of the first alternatives
to be examined is that of accessing the main memory less frequently
and making fewer additions.
A second alternative is to increase the ratio of row additions to row accesses.
The following algorithms will explore both choices.

The basic algorithm is straightforward in its implementation,
but it performs many additions of rows.  We present the following result.

\begin{lemma}
The cost in additions of the code
inside the innermost \textbf{for} loop is:
\[
   \left( \begin{array}{c} k \\ g \end{array} \right) ( g-1 ) n.
\]
\end{lemma}
\begin{proof}
The number of different combinations of $k$ rows taken $g$ rows at a time is
$\binom{k}{g}$.
For every one of those combinations, the algorithm performs $g-1$ row additions.
Every row addition consists of $n$ additions of bits.
By multiplying these three factors, the initial formula is obtained.
\end{proof}


% -----------------------------------------------------------------------------
\subsection{Optimized algorithm\label{alg:optimized_desc}}
% -----------------------------------------------------------------------------

In the basic algorithm presented above,
the order in which combinations are generated and processed
is not very important, except for cache effects.
On the other hand, in the optimized algorithm
the order in which the combinations are generated is more important,
since not all orders can help to reduce the number of additions.
The optimized algorithm will use the lexicographical order.
In this order, the indices in a combination change from the right-most part.
For instance, for 50 elements taken 3 elements at a time,
the combinations are generated in the following order:
$(0,1,2)$, $(0,1,3)$, $(0,1,4)$, $\ldots$, $(0,1,49)$,
$(0,2,3)$, $(0,2,4)$, $(0,2,5)$, $\ldots$, $(0,2,49)$,
$(0,3,4)$, $\ldots$

The advantage of the lexicographical order is that
each combination is very similar to the previous one.
In most cases of this order, there is only one difference between
one combination and the next one (or, equivalently, the previous one):
the last element.
Consequently,
in most cases the addition of the first $g-1$ rows performed
in one combination can be saved for the computation of the next combination,
thus saving many of them.
This method is outlined in Algorithm~\ref{alg:optimized}.


\begin{algorithm}[ht!]
  \caption{\ensuremath{\mbox{\sc Optimized algorithm}}}
  \label{alg:optimized}
  \begin{algorithmic}[1]
    \REQUIRE A generator matrix $G$ of the linear code $C$ with
             parameters $[n,k,d]$.
    \ENSURE  The minimum weight of $C$, i.e., $d$.
    \medskip
    \STATE \textbf{Beginning of Algorithm}
    \STATE [ $\Gamma_j$ ] = Compute\_gamma\_matrices( G );
    \FOR{ $g = 1, 2, \ldots$ }
      \FOR{ every $\Gamma$ matrix ($k \times n$) of $G$ }
        \STATE // Process all combinations of the $k$ rows of $\Gamma$ 
                  taken $g-1$ at a time:
        \STATE ( done, c ) = Get\_first\_combination();
        \WHILE{( ! done )}
          \STATE Process\_all\_combinations\_starting\_with( c, $\Gamma$ );
          \STATE ( done, c ) = Get\_next\_combination( c );
        \ENDWHILE
      \ENDFOR
    \ENDFOR
    \STATE \textbf{End of Algorithm}

    \medskip

    \STATE \textbf{Function} Get\_first\_combination() \textbf{is:}
    \STATE // Note that a combination contains $g-1$ indices in this algorithm.
    \STATE Return ( true, $(0,1,2,\ldots,g-2)$ )
    \STATE \textbf{End of Function}

    \medskip

    \STATE \textbf{Function} Get\_next\_combination( c ) \textbf{is:}
    \STATE done = Is\_this\_the\_last\_combination( c );
    \STATE c = Compute\_the\_next\_combination\_to\_be\_processed\_after( c );
    \STATE Return ( done, c )
    \STATE \textbf{End of Function}

    \medskip

    \STATE \textbf{Function} 
           Process\_all\_combinations\_starting\_with( c, $\Gamma$ ) 
           \textbf{is:}
    \STATE // Compute the addition of the $g-1$ rows of $\Gamma$ 
              with indices in c.
    \STATE // Generate all the combinations of $g$ rows 
              out of the combination prefix c with $g-1$ rows.
    \STATE // Generate all the additions of those combinations of $g$ rows
              by reusing the previous addition.
    \STATE // Compute the minimum weight of the additions of those combinations.
    \STATE // Update the lower and upper bounds, if needed.
    \STATE \textbf{End of Function}
  \end{algorithmic}
\end{algorithm}

The main structure of this algorithm is very similar to the basic one,
but there exist two major differences.
The first difference is that the combinations
are generated with $g-1$ elements instead of $g$ elements.
The second difference 
lies in the processing of the combinations.
The \texttt{Process\_all\_combinations\_starting\_with} function
receives a combination $c$ with $g-1$ elements,
then it adds the rows with indices in that combination
and, finally, it generates all the combinations of $g$ elements that start with
the received combination of $g-1$ elements by reusing the previous addition.
For instance, if $g=4$ and $c=(0,1,2)$,
it will first compute the additions of rows 0, 1, and 2,
and then it will reuse that addition to compute the
additions of the combinations $(0,1,2,3)$, $(0,1,2,4)$, \ldots, $(0,1,2,k-1)$,
thus saving $g-2$ (2 in this case) additions for every combination.

\begin{lemma}
The cost in additions of the code
inside the innermost \textbf{for} loop is:
\[
   \left[ \sum_{j=g}^{k-1} \left( \left( \begin{array}{c} j-2 \\ g-2 \end{array} \right)
                      ( g+k-j-1 ) \right) \right] n
\]
\end{lemma}
\begin{proof}
Assume that $c_i$ are the indices of the rows 
and assume that $c_{g-1}$ is set to the value $j$;
Then, we have $\binom{j-1}{g-2}$ different combinations
on the left part $(c_1, \ldots, c_{g-2})$.
Each of these different combinations require $g-2$ additions
and could be combined with any valid value of $c_{g}$ on the right part,
i.e., one has $k-j$ combinations.
So we have $\binom{j-1}{g-2}(g-2+k-j)$  additions.
Running through all the possible values of $j$, $j=g-1,\ldots, k-1$,
and considering $n$ bit additions per row we have:
\[
   \left[ \sum_{j=g}^{k-1} \left( \left( \begin{array}{c} j-2 \\ g-2 \end{array} \right)
                      ( g+k-j-1 ) \right) \right] n
\]

Modifying the initial index in the summation,
we get the initial formula.
\end{proof}


% -----------------------------------------------------------------------------
\subsection{Stack-based algorithm\label{alg:stack-based_desc}}
% -----------------------------------------------------------------------------

In the optimized algorithm,
the number of additions for every combination of $g-1$ rows
is always the same ($g-2$ additions)
since for every combination of $g-1$ rows
the addition of the rows is computed from scratch.
The additions of the desired combinations of $g$ rows
are built on top of those additions of $g-1$ rows
with just one extra addition for every combination of $g$ rows.

However, there are special orders (e.g.~the lexicographical order)
in which the current combination and the next one are usually similar.
If the current combination and the next one are similar,
some of the additions performed in the current combination 
could be reused to compute the additions required by the next combination.

In the stack-based algorithm,
the number of additions for every combination of $g-1$ rows
is reduced by using a stack and
generating the combinations in an orderly fashion.
The lexicographical order was used
because in this order the right-most elements change faster.
The stack must contain $g-1$ vectors of dimension $n$.
The memory used by this stack is not large at all
since both $n$ and $g$ are usually small,
and only one bit is needed for each element.
In most of our experiments, $n$ was always smaller than 300, and 
the algorithm usually finished for values of $g$ equal to or smaller than 16.
%%%% (Larger values of $g$ would require a very long time to finish:
%%%% months or even years of computation in a modern computer.)
Generally, the stack used less than 1 KByte of memory.
In addition, this stack can be reused for all $\Gamma_j$ matrices,
thus minimizing the overall space cost.

The stack works in an incremental way:
If a combination $c=(c_1,c_2,\ldots,c_{g-1})$, where $c_i$ is a row index
($c_i \in \{0,1,\ldots,k-1\}$),
is being processed,
the stack will contain the following elements (incremental additions):
row $c_1$,
the addition of rows $( c_1, c_2 )$,
the addition of rows $( c_1, c_2, c_3 )$,
\ldots,
and finally the addition of rows $( c_1, c_2, c_3, \cdots c_{g-1} )$.
Later, when a new combination is to be generated,
usually only the top elements of the stack (those with more additions)
must be recomputed.

An example is shown in Figure~\ref{figure:stack_example}.
Let us suppose that $k=50$, $g=6$, the current combination is $(0,1,2,3,48)$,
and therefore the next combination is $(0,1,2,4,5)$,
because combination $(0,1,2,3,49)$
cannot be combined with any other row to obtain a valid combination
of six elements (recall that $g=6$ in this example).
In the optimized algorithm, to process that next combination 
the addition of rows with indices $(0,1,2,4,5)$ should be computed,
that is, 4 rows would have to be added.
This number can be reduced by using a stack.
The contents of the stack for the current combination $(0,1,2,3,48)$
can be seen on the left side of the figure.
In that case, the stack contains the following elements:
row 1,
the addition of rows $( 0, 1 )$,
the addition of rows $( 0, 1, 2 )$,
the addition of rows $( 0, 1, 2, 3 )$, and finally 
the addition of rows $( 0, 1, 2, 3, 48 )$.
This last addition can be used to compute the desired combinations of $g$ rows.
Since the next combination is $(0,1,2,4,5)$,
instead of computing the addition of those rows from scratch (four additions),
the stack can be used (and updated at the same time) 
to compute the desired addition with only 2 additions
since only the two top elements must be updated.
The contents of the stack for the next combination $(0,1,2,4,5)$
can be seen on the right side of the figure.
%%%% As can be seen, the stack must be rebuilt
%%%% starting at the position of the left-most index that changes
%%%% from the current combination to the next one.

\begin{figure}[ht!]
\begin{center}
  \begin{tabular}{|c|c|c|c}
    \multicolumn{1}{c}{current combination = ( 0, 1, 2, 3, 48 )} & 
      \multicolumn{1}{c}{$\longrightarrow$} &
        \multicolumn{1}{c}{next combination = ( 0, 1, 2, 4, 5 )} & \\
    \multicolumn{1}{c}{} &
      \multicolumn{1}{c}{} &
        \multicolumn{1}{c}{} & \\ \cline{1-1} \cline{3-3}
    sum\_of\_rows( 0, 1, 2, 3, 48 ) &
      & 
        sum\_of\_rows( 0, 1, 2, 4, 5 ) & $\star$ \\ \cline{1-1} \cline{3-3}
    sum\_of\_rows( 0, 1, 2, 3 ) & 
      & 
        sum\_of\_rows( 0, 1, 2, 4 ) & $\star$ \\ \cline{1-1} \cline{3-3}
    sum\_of\_rows( 0, 1, 2 ) & 
      $\longrightarrow$ & 
        sum\_of\_rows( 0, 1, 2 ) & \\ \cline{1-1} \cline{3-3}
    sum\_of\_rows( 0, 1 ) & 
      & 
        sum\_of\_rows( 0, 1 ) & \\ \cline{1-1} \cline{3-3}
    sum\_of\_rows( 0 ) & 
      & 
        sum\_of\_rows( 0 ) & \\ \cline{1-1} \cline{3-3}
  \end{tabular}
\end{center}
%%%% \vspace*{-0.4cm}
\caption{Stack change when computing the next combination 
out of the current one.
Notice how only the top levels are changed (marked with $\star$),
thus reducing the number of additions.}
\label{figure:stack_example}
\end{figure}

The number of additions required to generate the next combination 
from the current combination depends on the left-most element
that will change from the current combination to the next one,
since the stack will have to be rebuilt from that level.
Hence,
to compute a combination of $g-1$ elements,
the minimum number of additions of the new algorithm is one, and
the maximum number of additions of the new algorithm is $g-2$.
Consequently,
to compute a combination of $g$ elements,
the minimum number of additions of the new algorithm is two, and
the maximum number of additions of the new algorithm is $g-1$.

The new stack-based method is outlined in Algorithm~\ref{alg:Stack}.
Notice how its structure is very similar to the previous one.
Now, there is a new function called \texttt{Create\_stack} that creates
the necessary data structures to hold the stack.
The remaining functions are modified to receive and in some cases 
return some additional arguments such as the stack and the $\Gamma$ matrix.
The \texttt{Get\_next\_combination} function rebuilds the stack,
and therefore it will require the stack as both an input argument and
an output argument.
It will also require the $\Gamma$ matrix as an input argument
to use the rows to update the stack.
On the other hand, 
the \texttt{Process\_all\_combinations\_starting\_with} function
uses the stack to compute the addition of the rows
performing fewer additions than the previous algorithm.


\begin{algorithm}[ht!]
  \caption{\ensuremath{\mbox{\sc Stack-based Algorithm}}}
  \label{alg:Stack}
  \begin{algorithmic}[1]
    \REQUIRE A generator matrix $G$ of the linear code $C$ with
             parameters $[n,k,d]$.
    \ENSURE The minimum weight of $C$, i.e., $d$.
    \medskip
    \STATE \textbf{Beginning of Algorithm}
    \STATE [ $\Gamma_j$ ] = Compute\_gamma\_matrices( G );
    \STATE stack = Create\_stack();
    \FOR{ $g = 1, 2, \ldots$ }
      \FOR{ every $\Gamma$ matrix ($k \times n$) of $G$ }
        \STATE // Process all combinations of the $k$ rows of $\Gamma$ 
                  taken $g-1$ at a time:
        \STATE ( done, c, stack ) = Get\_first\_combination( stack );
        \WHILE{ ( ! done ) }
          \STATE Process\_all\_combinations\_starting\_with( c, stack, $\Gamma$ );
          \STATE ( done, c, stack ) = Get\_next\_combination( c, stack, $\Gamma$ );
        \ENDWHILE
      \ENDFOR
    \ENDFOR
    \STATE \textbf{End of Algorithm}

    \medskip

    \STATE \textbf{Function} Get\_first\_combination( stack ) \textbf{is:}
    \STATE // Note that a combination contains $g-1$ indices in this algorithm.
    \STATE c = $(0,1,2,\ldots,g-2)$
    \STATE // Initialize stack with the contents of c.
    \STATE Return ( true, c, stack )
    \STATE \textbf{End of Function}

    \medskip

    \STATE \textbf{Function} Get\_next\_combination( c, stack, $\Gamma$ ) 
           \textbf{is:}
    \STATE done = Is\_this\_the\_last\_combination( c );
    \STATE c = Compute\_the\_next\_combination\_to\_be\_processed\_after( c );
    \STATE // Compare the new combination and the last one, 
    \STATE // and update the stack starting 
              at the left-most index with different contents.
    \STATE Return ( done, c, stack )
    \STATE \textbf{End of Function}

    \medskip

    \STATE \textbf{Function} 
           Process\_all\_combinations\_starting\_with( c, $\Gamma$ ) 
           \textbf{is:}
    \STATE // The top element of the stack contains 
              the addition of the $g-1$ rows of $\Gamma$ with indices in c.
    \STATE // Generate all the combinations of $g$ rows 
              out of the combination prefix c with $g-1$ rows.
    \STATE // Generate all the additions of those combinations of $g$ rows
              by reusing the previous addition.
    \STATE // Compute the minimum weight of the additions of those combinations.
    \STATE // Update the lower and upper bounds, if needed.
    \STATE \textbf{End of Function}
  \end{algorithmic}
\end{algorithm}


\begin{lemma}
The cost in additions of the code
inside the innermost \textbf{for} loop is:

\[
\left[  \left( \binom{k}{g}+\binom{k-1}{g-1}+\cdots+\binom{k-g+2}{2} \right)\right] n.
\]
\end{lemma}

\begin{proof}

We define the following sets of combinations for $i=1,\ldots,g-1$:
$$
B_i=\left\lbrace(c_1,\ldots,c_g)\mid c_g=c_{g-1}+1=c_{g-2}+2=\ldots=c_{g-i+1}+i-1\right\rbrace
$$
i.e., inside $B_i$ at least the last $i$ elements $(c_{g-i+1},\ldots,c_g)$ are consecutive.

Let us consider now a combination $(c_1,\ldots,c_g)$.
Assume that the last $r$ elements $(c_{g-r+1},\ldots,c_g)$ are consecutive,
but the last $r+1$ are not consecutive, i.e., $c_{g-r}+1\ne c_{g-r+1}$.
Then, the combination $(c_1,\ldots,c_g)$ requires no additions for the rows 
$(c_1,\ldots,c_{g-r})$ because the contents of the stack is reused.
However, $r$ additions are needed 
to update the higher levels of the stack with $(c_{g-r+1},\ldots,c_g)$.
So, we conclude that a combination with exactly $r$ consecutive elements at
the end requires $r$ additions.

The key observation is the following: a combination $(c_{1},\ldots,c_g)$
with exactly
 $r$ consecutive elements at the end is contained in exactly $r$ sets
$B_1,\ldots, B_r$.
Therefore, the number of additions required for a combination is equal to
the number of sets $B_i$ where it is contained.

We conclude that the total number of additions required is equal to the sum
of the cardinality of the sets $B_1,\ldots, B_{g-1}$.
So, in the rest of the proof we are going to calculate the cardinality of
these sets.

Notice that $B_1$ imposes no constrains, i.e., any combination
$(c_1,\ldots,c_g)$ is contained in $B_1$, therefore there are
$\binom{k}{g}$ elements in $B_1$.
Now we consider $B_2$.
A combination
$(c_1,\ldots,c_g)$  is in $B_2$ if and only if $c_g=c_{g-1}+1$.
This implies that when $(c_1,\ldots,c_{g-1})$ is fixed,
then $c_g$ is automatically fixed.
So, we have $\binom{k-1}{g-1}$ different combinations 
for $(c_1,\ldots,c_{g-1})$.
In general,  $(c_1,\ldots,c_g)$ is contained in $B_i$ if and only if
$c_g=c_{g-1}+1=c_{g-2}+2=\cdots=c_{g-i+1}+i-1$.
The latter condition implies that when $(c_1,\ldots,c_{g-i})$ is fixed,
then $(c_{g-i+1},\ldots,c_g)$ is automatically fixed.
So, we have $\binom{k-i}{g-i}$ possibilities for $(c_1,\ldots,c_{g-i})$.

Adding up the cardinals of $B_i$ for $i=1,\ldots, g-1$, we get
the following formula:
$\binom{k}{g}+\binom{k-1}{g-1}+\cdots+\binom{k-g+2}{2}$.
Finally, considering $n$ bit additions per row we get the stated formula
in this lemma.
\end{proof} 


% -----------------------------------------------------------------------------
\subsection{Algorithm with saved additions~\label{alg:stack-based-additions_desc}}
% -----------------------------------------------------------------------------

The basic algorithm performs $g-1$ additions
to process every generated combination.
The optimized algorithm performs only one addition in many cases,
and it performs $g-1$ additions in the remaining cases.
The stack-based algorithm performs only one addition in many cases,
and it performs between two and $g-1$ additions in the remaining cases.
Now we present an algorithm that performs the 
same low number of additions ($\ceil{g/s}$)
to process every generated combination.

The new algorithm always performs a fixed lower number of
additions for all combinations by using a larger additional storage.
Its main advantage is its smaller cost.
Its main disadvantage is the extra memory space needed,
but this issue is not a serious handicap,
since main memory in current computers is usually very large.

For every $\Gamma$ matrix, this algorithm saves 
the additions of all the combinations of
the $k$ rows taken $g$ at a time for values of $g = 1, 2, \ldots, s$
in the main memory.
The value $s$ is fixed at the beginning of the program,
and it determines the maximum amount of memory used.
In our experiments, we employed values of $s$ up to 5,
since it produced good performances 
and larger values required too much memory.
For instance, with $s=5$
this algorithm required a storage of around 95 MBytes
for processing the new linear codes presented in this paper,
which is not an excessive amount,
while producing good performances.

The saved additions of the combinations of $k$ rows
taken 1, 2, $\ldots$, $s$ rows at a time
will be then used to build the additions of the combinations of $k$ rows
taken $s+1$, $s+2$, $\ldots$ rows at a time.
This idea is simple, 
but the problem is to find a way to implement it 
that is sufficiently efficient.

If these additions are saved in the lexicographical order of the 
row indices in the combinations, it is efficient to combine them. 
This order is key to this algorithm.

This algorithm is to a certain extent similar to the stack-based algorithm.
The stack-based algorithm works on rows 
to compute combinations of rows on-the-fly 
by using the stack to reduce the cost.
In contrast,
the algorithm with saved additions first computes and saves combinations.
Then, once these combinations are saved,
this algorithm works on these saved combinations 
to generate the desired larger combinations.
In this case, the stack data structure does not explicitely exist,
but it is stored in the call stack of the process,
as local variables in each procedure call.

Next, we describe some details of the simplest case.
If $g = a + b$ with positive numbers $a$ and $b$ such that $a \leq s, b \leq s$,
the addition of the rows of the combination $c$ with indices
$(c_1, c_2, \ldots, c_{a}, c_{a+1} \ldots, c_{g})$
can be computed as the addition of the rows of the following combinations:
the combination $(c_1, c_2, \ldots, c_{a})$ (called left combination) and
the combination $(c_{a+1} \ldots, c_{g})$ (called right combination).
In this way, with just one addition the desired result can be obtained
if we have previously saved
the additions of the combinations of $k$ rows 
taken up to at least $\max(a,b)$ at a time.

Therefore, 
if $g = a + b$, to obtain the combinations of $k$ rows taken $g$ at a time,
the combinations of $k$ rows taken $a$ at a time (left combinations) and 
the combinations of $k$ rows taken $b$ at a time (right combinations)  
must be combined.
However, not all those combinations have to be processed.
There is one restriction to be applied to the left combinations,
and another one to be applied to the right combinations.
Next, both of them are described.
Note that it is very important that these restrictions must be applied
efficiently to accelerate this algorithm.
Otherwise, an important part of the performance gains could be lost.

In the case of the left combinations,
not all of the combinations have to be processed.
For instance, if $k=50$, $a=3$, and $b=2$,
left combinations starting with 46 or larger indices 
should be discarded
since no right combination can be appended to form a valid combination
(as an example, left combination $(46,47,48)$
cannot be concatenated to any right combination of two elements 
to form a valid combination).
If the saved additions of the combinations of $k$ elements taken $a$ at a time
are kept in the lexicographical order of the combinations, 
the following formula returns the index of the first combination 
in the saved combinations the processing of which must be avoided:

\[
   \left( \begin{array}{c} k     \\ a \end{array} \right) -
   \left( \begin{array}{c} g - 1 \\ a \end{array} \right)
\]

Likewise, in the case of the right combinations,
not all of the combinations have to be processed.
The last element in the left combination $(c_1, c_2, \ldots, c_{a})$ 
will define the right combinations with which this can be combined,
since 
it can only be combined with combinations starting with $c_{a}+1$ 
or larger values.
If the saved additions of the combinations are kept
in the lexicographical order of the combinations,
we can easily compute which combinations of $k$ rows taken $b$ at a time
must be processed.
The formula that returns the index of the first right combination 
to be combined is the following one, 
where $e$ is the last element in the left combination:

\[
   \left( \begin{array}{c} k         \\ b \end{array} \right) -
   \left( \begin{array}{c} k - e - 1 \\ b \end{array} \right)
\]

A general recursive algorithm that works for any $k$, any $g$, and any $s$ 
has been developed.
Recursive algorithms can be slow if
the computational cost inside every call is small 
in comparison to the call overhead,
but that is not our case.
In our algorithm the call overhead is negligible 
because the cost of the tasks performed inside each call is high,
and the maximum depth of the recursion is $\ceil{g/s}$.
The general method is outlined in Algorithm~\ref{alg:saved}.

The data structure that stores the saved additions
of the combinations of the rows of every $\Gamma$ matrix
must be built in an efficient way.
Otherwise, the algorithm could underperform for 
matrices that finish after only a few generators.
For every $\Gamma$ matrix, this data structure contains several 
levels ($l = 1, \ldots, s$),
where level $l$ contains all the combinations of the $k$ rows of the
$\Gamma$ matrix taken $l$ at a time.
The way to do it in an efficient way is 
to use the previous levels of the data structure to build the current level.
In our algorithms, 
to build level $l$, levels $l-1$ and $1$ were used.
This combination must be performed in a way that 
both keeps the lexicographical order in level $l$
and is efficient.

\begin{algorithm}[ht!]
  \caption{\ensuremath{\mbox{\sc Algorithm with Saved Additions}}}
  \label{alg:saved}
  \begin{algorithmic}[1]
    \REQUIRE A generator matrix $G$ of the linear code $C$ with
             parameters $[n,k,d]$.
    \ENSURE The minimum weight of $C$, i.~e., $d$.
    \medskip

    \STATE \textbf{Beginning of Algorithm}
    \STATE [ $\Gamma_j$ ] = Compute\_gamma\_matrices( G );
    \STATE Initialize\_data\_structures\_for\_storing\_additions( SA );
    \FOR{ $ g = 1, 2, \ldots $ }
      \FOR{ every $\Gamma_j$ matrix ($k \times n$) of $G$ }
        \IF{ $g \leq s$ }
          \STATE Generate and save all combinations of $g$ rows 
                 of $\Gamma_j$ into $\textrm{SA}_j$ ;
        \ENDIF
        \STATE Process\_step( $\textrm{SA}_j$, $g$, $\varnothing$ );
      \ENDFOR
    \ENDFOR
    \STATE \textbf{End of Algorithm}

    \medskip

    \STATE \textbf{Function} Process\_step( $\textrm{SA}_j$, $g$, $c$ ) 
           \textbf{is:}
    \STATE $ a = \min( g, s ) $;
    \STATE $ b = g - a $;
    \IF{ $ a < s $ }
      \STATE Compute the minimum distance of $\textrm{SA}_j$
             adding $c$ to suited combinations;
    \ELSE
      \FOR{ $j$ = index\_of( $k$, $a$, last\_element\_of( $c$ ) ) to
                  index\_of( $k$, $a$, $k - g$ ) }
        \STATE $e$ = $j$-th combination saved in $SA_j$;
        \IF{ $\textrm{last\_element\_of}( $e$ ) + b < k$}
          \STATE Process\_step( $\textrm{SA}_j$, $b$, $c + e$ );
        \ENDIF
      \ENDFOR
    \ENDIF
    \STATE \textbf{End of Function}

    \medskip

    \STATE \textbf{Function} index\_of( $p$, $q$, $r$ ) \textbf{is:}
    \STATE Return $\left( \begin{array}{c} p         \\ q \end{array} \right) - 
                   \left( \begin{array}{c} p - r - 1 \\ q \end{array} \right)$
    \STATE \textbf{End of Function}
  \end{algorithmic}
\end{algorithm}


\begin{lemma}
The cost in additions of the code
inside the loop in line 5 of Algorithm~\ref{alg:saved}
(equivalent part in the previous algorithms) is:
\[
  n \left[ \sum_{j = f \cdot s}^{ k -( g - f \cdot s)}
      \left( \binom{k-j}{g - s \cdot f} + f - 1 \right) 
      \cdot
      \binom{j-1}{f \cdot s-1} \right],
  \textrm{ where } f = \lfloor (g-1)/s \rfloor .
\]
\end{lemma}
\begin{proof}
Each combination $c$ contains $g$ elements.
As the algorithm saves combinations up to $s$ elements,
the $g$ elements must be partitioned into blocks of $s$ elements.
If $g$ is not a multiple of $s$, 
the last block will have less than $s$ elements.
The position of the next-to-last block is $f = \lfloor (g-1)/s \rfloor $.

As the first $f$ blocks always have $s$ elements,
in overall $f \cdot s$ combinations are evaluated.

The last element of the next-to-last block 
runs between $f \cdot s$ and $k - ( g - f \cdot s )$,
because the latter expression is the size of the last block.

Once the last element of the next-to-last block is fixed:
\[
  j = f \cdot s, \ldots, k - ( g - f \cdot s ) ,
\]
we have to choose the previous elements and the following elements
in the combination.
The previous elements can be chosen in: 
\[
  \binom{j-1}{f \cdot s-1},
\]
ways and the ways for the next elements are:
\[
  \binom{k-j}{g - s \cdot f} .
\]

For all the combinations ending in $j$, 
$f-1$ additions are performed for the previous blocks.
Therefore, the overall number of additions is:
\[
  \binom{j-1}{f \cdot s-1} \cdot ( f-1 ) .
\]

Moreover, for every one of the previous additions
an extra addition must be performed for 
all the combinations in the last block.
The number of possible choices for the last block is:
\[
  \binom{k-j}{g - s \cdot f} 
  \cdot
  \binom{j-1}{f \cdot s-1} .
\]

Performing summation over the above indices $j$, we obtain
the initial expression and the result follows.
\end{proof}

Although this algorithm performs much fewer additions than previous ones,
it has one drawback: 
the amount of data being stored and processed is much larger.
Even though the amount of data being stored is not prohibitive 
(around 50 MB in our experiments), 
the processing of those data will produce
many more cache misses than previous algorithms.
Recall that previous algorithms have to process just a few $\Gamma$ matrices
of dimension $k \times n$, 
whereas this algorithm must process a few matrices 
of dimension $ \left( \begin{array}{c} k \\ g \end{array} \right) \times n$,
for $g = 1,\ldots, s$.
In the first case, those few $\Gamma$ matrices can be stored in
the first levels of cache memory, 
whereas in the second case the matrices with the saved combinations 
will not usually fit there.


% -----------------------------------------------------------------------------
\subsection{Algorithm with saved additions and unrollings\label{alg:stack-based-additions-unroll_desc}}
% -----------------------------------------------------------------------------

All the algorithms described above perform $g-1$ row additions
for every $g$ row brought from the main memory,
the only difference among them being the number of total operations.
The goal of all of them, except the basic one,
is to reduce the total number of row additions and row accesses.
Since the ratio of row additions to row accesses is so low (close to one), 
and as the main memory is much slower than computing cores,
this low ratio might reduce performances 
when the memory system is especially slow or saturated.

We have developed
a variant of the algorithm with saved additions
that improves performance by increasing 
the ratio of additions to memory accesses,
in order to be less memory-bound.
The only difference is that
several combinations are processed at the same time,
and whenever one row is brought from the main memory, 
it will be reused as much as possible
in order to decrease the number of memory acceses.
This technique is called \textit{unrolling}, 
and it is widely used in high-performance computing.
This technique will reduce the number of times the memory is accessed,
and consequently the number of cache misses since
data are reused when transferred from the main memory.
In this unrolling scheme,
several combinations can be simultaneously computed,
because saved additions are only read, and not modified.
Therefore, there is no conflict between the processing 
of simultaneous combinations.

For instance,
by processing two combinations at the same time,
the number of rows accessed can be nearly halved
since each accessed row is used twice,
thus doubling the ratio of row additions to row acceses.
Processing three iterations at a time would improve this ratio
even further.
If more row additions per every row access are performed,
the fast computing cores will work closer to their limits, and
the main memory will cease to be a factor that limits performance.

In our experiments we have tested the processing of two combinations at a time,
and the processing of three combinations at a time.
We have not evaluated higher numbers because of the diminishing returns.

The loop in line 19 of algorithm~\ref{alg:saved} processes
one combination in each iteration of the loop.
To process two combinations at a time, this loop should be modified
to process two iterations of the old loop in each iteration of the new loop.

But executing two or more iterations at a time 
is more effective when their last elements are exactly the same.
When the last element is the same, both left combinations must be
combined with the same subset of right combinations.
In contrast, when the last element is different, 
each left combination must be combined 
with a different subset, and therefore it is not so effective to blend them.
For instance, left combinations $(0,1,4)$ and $(0,2,4)$ can be executed
at the same time, 
whereas in left combinations $(0,1,2)$ and $(0,1,3)$ 
the blending is not so effective.

If the lexicographical order is employed,
the last element of the combinations is the one that changes most.
In this case, 
consecutive combinations usually contain different final elements,
and the unrolling will not be so effective.
Therefore, a new order must be used.
The requirements for this new order are two-fold:
The first one is that 
the left-most element must be the one that changes least
so that we can efficiently access all combinations starting with
some given element (the last one of the previous combination plus one).
The second one is that the right-most element must change very little,
in order to be able to blend as many consecutive combinations as possible.
Hence, the order we have used is a variation of the lexicographical
one in which the element that changes least is the first one,
then the last one, and then the rest.
For instance, if $k=5$ and $g=3$, 
the order is the following one:
$(0,1,2)$,
$(0,1,3)$,
$(0,2,3)$,
$(0,1,4)$,
$(0,2,4)$,
$(0,3,4)$,
etc.


% -----------------------------------------------------------------------------
\subsection{Cost comparison}
% -----------------------------------------------------------------------------

The cost of each algorithm has been previously shown;
for the brute-force algorithm the overall cost was given, and
for the rest of the algorithms, based on Brouwer-Zimmermann,
only the cost of the innermost loop was given
since the number of iterations in the $g$ loop is unknown
due to the fact that it is able to terminate earlier.
Since those formulae are complex, it is difficult to compare them
and to extract conclusions.
Table~\ref{table:cost-comparison} shows the costs 
of the algorithms based on Brouwer-Zimmermann 
for several values of $g$ for both $k=50$ and $k=75$. 
The factor $n$ is not considered since it appeared in all the formulae.
The cost of the algorithm with saved additions is computed considering $s=5$.
This table shows the rounded number of operations in billions ($10^9$).
As can be seen, each algorithm is faster than the one above.
The improvement between the first one and the best one is considerable.
These results were similar to those obtained in the experimental section,
despite the fact that additions were the only operations considered.

\begin{table}[htbp]
\begin{center}
\begin{tabular}{l@{\hskip 0.5cm}rrrr@{\hskip 0.5cm}rrrr} \toprule
  &
  \multicolumn{4}{c}{$k=50$} &
  \multicolumn{4}{c}{$k=75$} \\
  Algorithm & 
  \multicolumn{1}{c}{$g=7$} &
  \multicolumn{1}{c}{$g=10$} & 
  \multicolumn{1}{c}{$g=15$} & 
  \multicolumn{1}{c}{$g=20$} & 
  \multicolumn{1}{c}{$g=7$} & 
  \multicolumn{1}{c}{$g=10$} & 
  \multicolumn{1}{c}{$g=15$} & 
  \multicolumn{1}{c}{$g=20$} \\ \midrule
  Basic       & 0.599 & 92.50 & 31520.0 & 894976.0 & 11.90 & 7464.0 & 31916032.0 &  15267266560.0 \\
  Optimized   & 0.170 & 26.71 & 11029.1 & 386459.5 &  2.91 & 1713.1 &  8208045.7 &   4658374391.3 \\
  Stack-based & 0.116 & 12.78 &  3188.7 &  77535.2 &  2.18 &  954.5 &  2840671.5 &   1090013712.2 \\
  Saved       & 0.100 & 10.27 &  2254.0 &  47818.9 &  1.98 &  828.9 &  2280409.4 &   804610959.9 \\
  \bottomrule
\end{tabular}
\end{center}
\vspace*{0.1cm}
\caption{Rounded number of additions in billions ($10^9$)
in the innermost loop for $k=50$ (left) and $k=75$ (right) 
and several values of $g$.
The cost of the saved algorithm was computed considering $s=5$.}
\label{table:cost-comparison}
\end{table}



==> old/crc_tex_toms_rev2/4_Implementation.tex <==
% =============================================================================
\section{Implementation and optimization details}
\label{sec:implementation_and_optimization}
% =============================================================================


% -----------------------------------------------------------------------------
\subsection{Parallelization of the brute-force algorithm 
            with Gray code based enumeration}
% -----------------------------------------------------------------------------

The parallelization of the brute-force algorithm 
with Gray code based enumeration (Algorithm~\ref{alg:gray-code-brute-force})
is straightforward.
Its main loop (line 2) can be easily parallelized
by partitioning iterations between the threads,
and assigning one thread to every core.
Since the cost of all iterations is very homogeneous,
a static scheduling is enough to obtain high performances.
However, not every static scheduling is optimal in this case.
To take full advantage of the Gray code based enumeration,
a block partitioning of the iterations between the threads must be used
since this partitioning assigns consecutive iterations to the same thread.
Other partitionings (e.g.~cyclic partitioning) should be discarded
because the ranges of iterations assigned to every thread are not contiguous.
Just a small critical section must be used 
to concurrently update the minimum distance.
However, the impact of this critical section can be minimized 
by making every thread work with a local distance, and 
by updating the global distance just once at the end.


% -----------------------------------------------------------------------------
\subsection{Parallelization of the basic algorithm}
% -----------------------------------------------------------------------------

The parallelization of
the outer loop \texttt{For g} (line 3 of Algorithm~\ref{alg:basic}) 
is very challenging because it should be recalled that 
the iterative process can finish after any iteration of this loop
(whenever the minimum weight is larger than some value).
Hence, executing several iterations of this loop at the same time
could initiate the processing of iterations that are not really needed.
Besides,
it will not produce high performances
since the number of iterations of this loop 
can be smaller than the number of cores.
For instance, in our experiments 
the number $g$ was always equal to or smaller than 16, 
and the maximum number of cores was 28.
As the number of cores can be much higher than the highest $g$,
the parallelization of this loop 
would not take advantage of all the computer power.
In addition,
the cost of every iteration of the $g$ loop varies a great deal
(the cost of each iteration is usually higher than 
the addition of the cost of all the previous iterations).
Because of all of these causes, the parallelization of this loop 
must be discarded.

The middle loop \texttt{For every $\Gamma$} 
(line 4 of Algorithm~\ref{alg:basic}) 
can be easily parallelized
(by assigning a different $\Gamma$ matrix to every core).
Despite the cost of processing every $\Gamma$ matrix is very similar,
in order to be able to parallelize this algorithm
there should be as many or more $\Gamma$ matrices than computing cores,
but that is not usually the case.
For example, in our most time-consuming experiments 
there were 5 $\Gamma$ matrices,
whereas current computers can have a higher number of cores.
So this solution must also be discarded due to its inefficiency and
lack of potential scalability.

The \texttt{while} loop (line 7 of Algorithm~\ref{alg:basic}) 
can be easily parallelized with a dynamic scheduling,
but it has an important drawback that 
makes the parallelization inefficient:
The invocation of \texttt{Get\_next\_combination} (line 7) should be inside a
critical region so that only one thread can execute this method at a time.
Otherwise, two threads could get the same combination or, worse yet,
one combination could be skipped.
%
This parallelization strategy works fine 
for a very low number of threads (about two or three),
but when using more threads,
the method \texttt{Get\_next\_combination} becomes a big bottleneck,
and performances drop significantly.
%
Another approach would be the parallelization of the \texttt{while} loop 
with a static scheduling.
To do that, the first and last combinations for every thread should
be computed easily and quickly before starting it.
Since we have not found a cheap way to achieve it and 
the cost of this algorithm is much higher than the cost of other algorithms,
there is not much point in pursuing this.

In conclusion,
despite the simplicity of the structure of the basic algorithm,
its parallelization will not usually produce high performances.


% -----------------------------------------------------------------------------
\subsection{Parallelization of the optimized algorithm}
% -----------------------------------------------------------------------------

As the structure of the optimized algorithm is so similar to the
structure of the basic algorithm,
its parallelization is going to present the same drawbacks.
Although 
the concurrent method \texttt{Process\_all\_combinations\_starting\_with}
has a higher cost than the analogous one of the previous algorithm, 
the critical region in method \texttt{Get\_next\_combination} 
would make performances drop when the number of cores is slightly higher.
Therefore, the parallelization of this algorithm must be discarded too.


% -----------------------------------------------------------------------------
\subsection{Parallelization of the stack-based algorithm}
% -----------------------------------------------------------------------------

The structure of the stack-based algorithm is very similar to the previous one,
and therefore it has the same drawbacks.
The main difference between this one and the optimized algorithm is 
that the cost of the method \texttt{Get\_next\_combination} is higher
since the stack must be rebuilt in some cases.
This fact makes the parallelization of this algorithm even less appropiate 
since the cost of the critical region is higher.


% -----------------------------------------------------------------------------
\subsection{Parallelization of the algorithms with saved additions}
% -----------------------------------------------------------------------------

The structures of 
the algorithm with saved additions
and the algorithm with saved additions and unrollings
are very similar.
So, both of them will be tackled at the same time.

The parallelization of the algorithms with saved additions
is very different from the previous ones.
As the combinations are already generated and 
the additions of those are saved in vectors,
its parallelization does not require the use of a large critical section,
thus producing higher potential gains in the parallel implementations.
The loop that must be parallelized is the \texttt{for} loop of the
\texttt{else} branch
(line 19 of Algorithm~\ref{alg:saved}),
but it must only be parallelized for the first level of the recursion.
Hence, we have an algorithm, the algorithm with saved additions,
that is both efficient and parallel.

In the parallelization of this loop of this algorithm,
a dynamic scheduling strategy must be used
since the cost of processing every element of the vector 
(subcombination) is very different.
For instance, if $k=50, g=6, s=3$,
processing iteration $(0,1,2)$ would require much longer than 
processing iteration $(0,1,46)$.
In the first case, many combinations must be processed:
$(0,1,2,3,4,5)$, $(0,1,2,3,4,6)$, \ldots.
In the second case, the only combination to be processed would be:
$(0,1,46,47,48,49)$.
In our parallelized codes, we used OpenMP~\cite{OpenMP} to achieve
the dynamic scheduling strategy of mapping loop iterations to cores.

We used a small critical section for updating the overall minimum weight.
However, we minimized the impact of this critical section by making
every thread work with local variables, and by updating the global
variables just once at the end.


% -----------------------------------------------------------------------------
\subsection{Vectorization and other implementation details}
% -----------------------------------------------------------------------------

Usual scalar instructions process
one byte, one integer, one float, etc.\ at a time.
In contrast, hardware vector instructions make it possible 
to process many numbers at a time, thus improving performances.
Vector instructions use vector registers,
whose size depends on the architecture.
For example, whereas older x86 architectures used 128-bit registers
(Intel's SSE --Streaming SIMD Extensions--), 
modern architectures use 256-bit (AVX --Advanced Vector Extensions--)
or even 512-bit registers (--AVX-512 extensions--).
With so wide vector registers, 
just one vector instruction can process a considerable number of elements.

However, one drawback of the vector instructions is its standardization.
Every new architecture contributes new vector instructions,
and older architectures do not support the new vector instructions.
Therefore, developing a vector code is not straightforward because it will
depend on the architecture.

One of the commercial and most widely employed implementations, \magma{},
only allows the use of hardware vector instructions 
on the newest architectures with AVX support, 
and does not support vectorization on processors with SSE.
Unlike \magma{}, our implementations are more flexible,
and they can use hardware vector instructions
both in processors with SSE, AVX or AVX-512 support,
that is, in both old and new processors, both from Intel and AMD.

Another serious challenge in the vectorization is the low number of elements
since the length $n$ is usually smaller than a few hundreds.
In general, vectorization requires a very high number of elements 
to be faster than the equivalent scalar codes.


% -----------------------------------------------------------------------------
%\subsection{Other Implementation Details}
% -----------------------------------------------------------------------------

When developing a high-performance implementation,
the algorithm is very important,
but even then some small implementation choices can greatly affect 
the performances.

We used the C language since it is a compiled language, 
and therefore it usually produces high performances.
We have also chosen it because of its high portability.

In our implementations, we used the 32-bit integer as the basic datatype,
thus packing 32 elements into each integer.
This provides high performances for the scalar implementations
since just one scalar instruction can process up to 32 elements.

We also tested 64-bit integers since in one operation more elements 
would be processed.
When the performances obtained using 32-bit integers and
those obtained using 64-bit integers were compared,
the results depended on the architecture and on the number of columns 
of the code.
%
On the one hand,
for codes with many columns, 
using 64-bit integers produced somewhat higher performances.
On the other hand, 
for codes with a small number of columns,
using 32-bit integers clearly produced higher performances.
Since vectorization is much faster when there are many columns,
we decided to use 32-bit integers.
%
We think that the cause of this drop when using 64-bit integers 
on codes with few columns
is the fact that additional elements that must be processed (and stored)
when $n$ is not a multiple of the number of bits of the basic datatype.
When 64-bit integers are used,
$64 \lceil(n/64)\rceil - n$ additional elements must be processed.
On the other hand, 
when 32-bit integers are used,
$32 \lceil(n/32)\rceil - n$ additional elements must be processed,
which is usually a smaller overhead.



==> old/crc_tex_toms_rev2/5_Performances.tex <==
% =============================================================================
\section{Performance analysis}
\label{sec:performance_analysis}
% =============================================================================

This section describes and analyizes the performance results 
attained by our implementations,
comparing them with state-of-the-art software that perform the same tasks.
The experiments reported in this article were performed 
on the following two computing platforms:

\begin{itemize}

\item
\texttt{Cplex}: 
This computer was based on AMD processors.
It featured an AMD Opteron\texttrademark\ Processor 6128 (2.0 GHz), 
with 8 cores.
Its OS was GNU/Linux (Version 3.13.0-68-generic).
Gcc compiler (version 4.8.4) was used.
In the experiments we usually used up to 6 cores (of the 8 cores it had)
since we were not the only users.
Note that some of the experiments presented in this section lasted for weeks.

\item
\texttt{Marbore}: 
This computer was based on Intel processors.
It featured two Intel Xeon\circledR\ CPUs E5-2695 v3 (2.30 GHz), 
with 28 cores in total.
Its OS was GNU/Linux (Version 2.6.32-504.el6.x86\_64).
Gcc compiler (version 4.4.7) was used.
As this was a dedicated computer, we used all its cores in the experiments.
In this computer the so-called {\em Turbo Boost} mode of the CPU was turned off
in our experiments.

\end{itemize}

Our implementations were compared with 
the two most-common implementations currently available:

\begin{itemize}

\item
\magma{}~\cite{Magma}:
It is a commercial software package designed for computations in algebra,
algebraic combinatorics, algebraic geometry, etc.
Version 2.22-3 was employed in our experiments.
Given the limitations in its commercial license,
it was available only in the AMD computer,
and it was not in the Intel computer.

As \magma{} only allows the use of hardware vector instructions 
on the newest processors with AVX support, and not on processors with SSE,
we could not use this feature in the AMD computer.
Therefore, the version of \magma{} we evaluated only used scalar instructions.
We evaluated \magma{} on both serial and multiple cores 
since it allows the user to define the number of cores to be used
on multi-core architectures.

On the contrary, our implementations are more flexible,
and they can use hardware vector instructions
both on processors with SSE and AVX support,
that is, on both old and new processors, both from Intel and AMD.

\item
\guava{}~\cite{GAP,Guava}:
GAP (\textit{Groups, Algorithms, Programming}) is a software environment
for working on computational discrete algebra and computational group theory.
It includes a package named \guava{} that contains software to compute 
the minimum weight of linear codes.
\guava{} Version 3.12 and GAP Version 4.7.8 were employed in our experiments.
It was installed on both computer platforms.

\guava{} does not allow the use of hardware vector instructions,
and therefore it uses only scalar instructions.
Moreover, it does not allow the use of multiple cores,
and therefore it was evaluated on only one core.
Hence, \guava{} was evaluated only on one core of both architectures
with scalar instructions.

Unlike \guava{}, our implementations can use 
both scalar and hardware vector instructions,
both on one and on several cores.

\end{itemize}

In subsection~\ref{sec:bz} we will compare the 
algorithms described in this paper based on Brouwer-Zimmermann method
to determine the best one.
In subsection~\ref{sec:bfbz} we will compare the 
best implementation of the brute-force algorithm (Gray code based enumeration) 
and the best algorithm based on Brouwer-Zimmermann method.
In subsection~\ref{sec:onecore} we will compare the 
best implementations developed in this paper 
and the implementations currently available on one core.
In subsection~\ref{sec:multicores} we will compare the 
best implementations developed in this paper 
and the implementations currently available on multicore machines.
In subsection~\ref{sec:parallelization} we will explore the scalability and 
parallel performance of our new implementations.


% -----------------------------------------------------------------------------
\subsection{A comparison of the algorithms based 
            on the Brouwer-Zimmermann algorithm~\label{sec:bz}}
% -----------------------------------------------------------------------------

Table~\ref{table:inside} reports the time spent by the algorithms 
to compute the minimum distance of 
a random linear code with parameters [150,50,28].
As can be seen, the performances are very encouraging since
the best algorithm is more than 6 times as fast as the worst one.
This improvement reflects the qualities and virtues of some of our algorithms.
The optimized algorithm improves the performances of the basic one 
since it performs fewer additions.
The stack-based algorithm again improves the performances of the optimized one 
since it performs even fewer additions.
The method based on saving combinations performs even fewer additions
by saving and reusing previous additions, and thus it produces higher 
performances.
The algorithm with saved additions and unrollings performs exactly the
same additions as the algorithm with saved additions,
but it accesses the memory fewer times,
thus attaining better performances in one of the two computers:
the one with the slowest memory system.
For larger codes the performances of the last algorithm were even better 
than those shown in the table, since the number of saved data was larger
and the memory started to become a serious bottleneck.


\begin{table}[ht!]
\vspace*{0.4cm}
\begin{center}
\begin{tabular}{lrr}
	\toprule
  \multicolumn{1}{c}{Implementation} & 
  \multicolumn{1}{c}{\texttt{cplex}} & 
  \multicolumn{1}{c}{\texttt{marbore}} \\ \midrule
  Basic                                          & 511.5 & 273.1 \\
  Optimized                                      & 191.0 & 105.3 \\ 
  Stack-based                                    & 144.5 &  84.6 \\ 
  Saved additions with $s=5$                     &  89.8 &  44.7 \\ 
  Saved additions with $s=5$ and unrollings by 2 &  74.0 &  44.6 \\ 
  \bottomrule
\end{tabular}
\end{center}
\caption{Time (in seconds) for the different implementations
         on a linear code with parameters [150,50,28].}
\label{table:inside}
\end{table}


% -----------------------------------------------------------------------------
\subsection{A comparison of the brute-force algorithm and
            the best algorithm based on Brouwer-Zimmermann~\label{sec:bfbz}}
% -----------------------------------------------------------------------------

Figure~\ref{figure:gray-saved} shows the time in seconds
obtained by two algorithms:
the brute-force algorithm with Gray code based enumeration 
and the algorithm with saved additions.
Both algorithms have been evaluated on one core of \texttt{marbore}
with scalar instructions (no vector machine instructions).
Two different types of codes have been used:
The left panel shows the results obtained for nearly square codes 
($k \approx n$),
whereas the right panel shows the results obtained for very rectangular codes 
($k \ll n = 512$).

\begin{figure}[ht!]
\vspace*{0.4cm}
\begin{center}
\begin{tabular}{cc}
\includegraphics[width=0.48\textwidth]{plots/time_line_gray_saved/time_line_gray_saved_square_marbore_1c} &
\includegraphics[width=0.48\textwidth]{plots/time_line_gray_saved/time_line_gray_saved_512xk_marbore_1c} \\
\end{tabular}
\end{center}
\vspace*{-0.4cm}
\caption{Time in seconds
for the brute-force algorithm with Gray code based enumeration
and the algorithm with saved additions 
on one core of \texttt{marbore}
for two different types of codes 
(nearly square on the left; very rectangular on the right).}
\label{figure:gray-saved}
\end{figure}

On nearly square codes, 
the Gray code based enumeration produces better performances on small codes 
since it is very simple and no $\Gamma$ matrices have to be built.
However, as the dimension and length of the codes grow,
the algorithm with saved additions produces much higher performances
(several orders of magnitude) 
due to the fact that it can terminate much earlier.
The threshold value is about 15 in this case, 
but it depends on the architecture.

On very rectangular codes,
the Gray code based enumeration produces better performances 
on small values of $k$ again,
and the algorithm with saved additions produces much higher performances
when $k$ grows.
The threshold value is about 27 in this case,
and the performance differences are smaller.

These results show that the brute-force algorithm 
with Gray code based enumeration
can be faster on small values of $k$.
The exact threshold depends on the architecture and 
also on the dimension $n$.
In any other cases, the algorithm with saved additions,
based on Brouwer-Zimmermann, should be used.


% -----------------------------------------------------------------------------
\subsection{A comparison of the best implementations 
            on one core~\label{sec:onecore}}
% -----------------------------------------------------------------------------

Table~\ref{table:singlecore1} compares our best implementations
and the two best implementations available, \magma{} and \guava{},
for some linear codes of medium size on one core of \texttt{cplex}.
We do not include the brute-force algorithm since 
it can be very slow for high values of $k$, as was shown.

As \magma{} cannot use hardware vector instructions in the computer 
used in the experiments,
we could only evaluate it with scalar instructions.
As \guava{} cannot use hardware vector instructions at all,
we could only evaluate it with scalar instructions.
%
We show two implementations of our best algorithm:
the first one uses only scalar instructions, 
and the second one uses hardware vector instructions.

Both of our new implementations clearly outperform the other two in all cases.
Our new implementations are several times faster than the current ones.
The performance improvement is remarkable in these cases: 
Our scalar implementation is on average 3.00 times as fast as \magma{}, and
our vector implementation is on average 5.36 times as fast as \magma{}.
Our scalar implementation is on average 4.36 times as fast as \guava{}, and
our vector implementation is on average 8.09 times as fast as \guava{}.


\begin{table}[ht!]
\vspace*{0.4cm}
\begin{center}
\begin{tabular}{crrrr}
	\toprule
    \multicolumn{1}{c}{Code} & 
    \multicolumn{1}{c}{\magma{}} & 
    \multicolumn{1}{c}{\guava{}} & 
    \multicolumn{1}{c}{Scalar Saved} & 
    \multicolumn{1}{c}{Vector Saved} \\ \midrule
  $[150,50,28]$ &     161.1 &     193.6 &      74.0 &      38.9 \\  
  $[130,67,15]$ &   1,980.0 &   1,585.5 &     574.8 &     331.3 \\  
  $[150,50,34]$ &   4,590.8 &  33,845.9 &   2,594.4 &   1,344.0 \\  
  $[115,63,11]$ &   5,056.7 &   3,703.7 &   1,292.8 &     755.1 \\  
  $[102,62,12]$ &  20,585.9 &  14,356.8 &   5,258.0 &   3,047.5 \\  
  $[150,77,17]$ &  53,052.9 &  40,804.3 &  19,262.2 &  10,245.4 \\  
    \bottomrule
\end{tabular}
\end{center}
\caption{Time (in seconds) for the best implementations
         on several linear codes of medium size 
         on one core of \texttt{cplex}.}
\label{table:singlecore1}
\end{table}


Table~\ref{table:singlecore3} compares the implementations 
for the new linear codes 
on one core of \texttt{cplex}.
These linear codes are larger than the previous linear codes.
Our two new implementations clearly outperform 
the usual current implementations.
Our scalar implementation is on average 1.81 times as fast as \magma{}, and
our vector implementation is on average 3.77 times as fast as \magma{}.
Our scalar implementation is on average 1.77 times as fast as \guava{}, and
our vector implementation is on average 3.69 times as fast as \guava{}.


\begin{table}[ht!]
\vspace*{0.4cm}
\begin{center}
\begin{tabular}{crrrr}
	\toprule
    \multicolumn{1}{c}{Code} & 
    \multicolumn{1}{c}{\magma{}} & 
    \multicolumn{1}{c}{\guava{}} & 
    \multicolumn{1}{c}{Scalar Saved} & 
    \multicolumn{1}{c}{Vector Saved} \\ \midrule
  $[235,51,64]$ & 802,364.2 & 681,339.1 & 484,788.1 & 234,890.8 \\ 
  $[236,51,64]$ & 786,181.6 & 686,686.4 & 484,834.9 & 231,345.5 \\ 
  $[233,51,62]$ & 643,663.4 & 567,629.1 & 335,678.6 & 159,470.8 \\ 
  $[233,52,61]$ & 687,073.4 & 934,105.0 & 359,489.1 & 173,112.4 \\ 
  $[232,51,61]$ & 503,984.2 & 456,413.2 & 261,250.3 & 125,695.6 \\ 
    \bottomrule
\end{tabular}
\end{center}
\caption{Time (in seconds) for the best implementations
         on the new linear codes 
         on one core of \texttt{cplex}.}
\label{table:singlecore3}
\end{table}


Figure~\ref{figure:singlecore1} shows 
the performances (in terms of combinations per second)
for all the linear codes on one core of \texttt{cplex}.
Therefore, the higher the bars, the better the performances are.
The total number of combinations processed by all the algorithms 
are usually similar, but not identical, 
since some algorithms (such as \guava{}) 
can process an additional $\Gamma$ matrix in a few cases.
To make the comparison fair, all the algorithms used the same
total number of combinations: those returned by \guava{}.
This figure shows that 
both the new scalar and vector implementations clearly outperform 
both \magma{} and \guava{} for all cases.

\begin{figure}[ht!]
\vspace*{0.4cm}
\begin{center}
\begin{tabular}{cc}
\includegraphics[width=0.48\textwidth]{plots/cps_bar/cps_bar_med_cplex_1c} &
\includegraphics[width=0.48\textwidth]{plots/cps_bar/cps_bar_lar_cplex_1c}
\end{tabular}
\end{center}
\vspace*{-0.4cm}
\caption{Performance (in terms of $10^{6}$ combinations per sec.) 
         of the best implementations for all the linear codes
         on one core of \texttt{cplex}.}
\label{figure:singlecore1}
\end{figure}


% -----------------------------------------------------------------------------
\subsection{A comparison of the best implementations 
            on multicores~\label{sec:multicores}}
% -----------------------------------------------------------------------------

Table~\ref{table:multicore1} compares our best implementations
and the best implementations available 
for some linear codes of medium size on multiple cores of \texttt{cplex}.

As \guava{} cannot use several cores, it was not included in these experiments.
As \magma{} cannot use hardware vector instructions in the computer being used,
we could only evaluate it with scalar instructions.

The performance improvement is also remarkable in these cases: 
Our new implementations are several times faster than \magma{}.
Our scalar implementation is on average 3.01 times as fast as \magma{}, and
our vector implementation is on average 5.21 times as fast as \magma{}.
The improvement factors of our new implementations in comparison to \magma{}
on multicores are similar to those on a single core,
thus showing that our parallelization is as good as that of \magma{}.


\begin{table}[ht!]
\vspace*{0.4cm}
\begin{center}
\begin{tabular}{crrr}
	\toprule
    \multicolumn{1}{c}{Code} & 
    \multicolumn{1}{c}{\magma{}} & 
    \multicolumn{1}{c}{Scalar Saved} & 
    \multicolumn{1}{c}{Vector Saved} \\ \midrule
  $[150,50,28]$ &      29.3 &      13.5 &       7.8 \\ 
  $[130,67,15]$ &     345.3 &     104.7 &      64.9 \\ 
  $[150,50,34]$ &     771.6 &     435.5 &     228.9 \\ 
  $[115,63,11]$ &     860.5 &     224.4 &     134.2 \\ 
  $[102,62,12]$ &   3,659.8 &     894.7 &     525.1 \\ 
  $[150,77,17]$ &   9,562.8 &   3,314.6 &   1,763.1 \\ 
    \bottomrule
\end{tabular}
\end{center}
\caption{Time (in seconds) for the best implementations
         on several linear codes of medium size
         on 6 cores of \texttt{cplex}.}
\label{table:multicore1}
\end{table}


Table~\ref{table:multicore3} compares our best implementations
and the best implementations available 
for the new linear codes 
on multiple cores of \texttt{cplex}.
The performance improvement is also remarkable in these cases: 
Our new implementations are faster than \magma{}.
On average,
our scalar implementation is 1.82 times as fast as \magma{}, and
our vector implementation is 3.82 times as fast as \magma{}.
The improvement factors of our new implementations in comparison to \magma{}
on multicore are also similar to those on a single core.


\begin{table}[ht!]
\vspace*{0.4cm}
\begin{center}
\begin{tabular}{crrr}
	\toprule
    \multicolumn{1}{c}{Code} & 
    \multicolumn{1}{c}{\magma{}} & 
    \multicolumn{1}{c}{Scalar Saved} & 
    \multicolumn{1}{c}{Vector Saved} \\ \midrule
  $[235,51,64]$ & 133,233.3 &  80,963.0 &  38,428.5 \\ 
  $[236,51,64]$ & 132,385.7 &  80,966.6 &  38,497.1 \\ 
  $[233,51,62]$ & 108,552.2 &  56,083.6 &  26,725.6 \\ 
  $[233,52,61]$ & 116,002.6 &  60,124.6 &  28,812.9 \\ 
  $[232,51,61]$ &  85,341.1 &  43,618.6 &  20,691.6 \\ 
	\bottomrule
\end{tabular}
\end{center}
\caption{Time (in seconds) for the best implementations
         on the new linear codes
         on 6 cores of \texttt{cplex}.}
\label{table:multicore3}
\end{table}

Figure~\ref{figure:multicore1} shows 
the performances (in terms of combinations per second)
for all the linear codes on 6 cores of \texttt{cplex}.
Therefore, the higher the bars, the better the performances are.
To make the comparison fair, all the algorithms used the same
total number of combinations: those returned by \guava{}.
This figure shows that 
both the new multicore scalar and vector implementations clearly outperform 
\magma{} for all cases.

\begin{figure}[ht!]
\vspace*{0.4cm}
\begin{center}
\begin{tabular}{cc}
\includegraphics[width=0.48\textwidth]{plots/cps_bar/cps_bar_med_cplex_6c} &
\includegraphics[width=0.48\textwidth]{plots/cps_bar/cps_bar_lar_cplex_6c}
\end{tabular}
\end{center}
\vspace*{-0.4cm}
\caption{Performance (in terms of $10^{6}$ combinations per sec.) 
         of the best implementations for all the linear codes
         on 6 cores of \texttt{cplex}.}
\label{figure:multicore1}
\end{figure}


% -----------------------------------------------------------------------------
\subsection{Parallelization and scalability~\label{sec:parallelization}}
% -----------------------------------------------------------------------------

Figure~\ref{figure:scal1} shows the speedups obtained by both 
our scalar and vector algorithms with saved additions 
for several configurations of cores 
on both \texttt{cplex} and \texttt{marbore}.
We employed a medium-sized code with parameters [150,77,17], and 
similar results were obtained on other codes.
In these cases, we used up to all the 8 cores in \texttt{cplex}.
The two plots show that the new implementations are remarkably scalable,
even with a high number of cores, 
since the speedups obtained are very close to the perfect ones.
For instance, when run on the 28 cores of \texttt{marbore},
the parallel implementation was more than 26 times as fast as 
the serial implementation.

\begin{figure}[ht!]
\vspace*{0.4cm}
\begin{center}
\begin{tabular}{cc}
\includegraphics[width=0.48\textwidth]{plots/scalability/scal_cplex} &
\includegraphics[width=0.48\textwidth]{plots/scalability/scal_marbore}
\end{tabular}
\end{center}
\vspace*{-0.4cm}
\caption{Speedups obtained on both machines 
         (\texttt{cplex} left; \texttt{marbore} right).}
\label{figure:scal1}
\end{figure}




==> old/crc_tex_toms_rev2/6_New_linear_codes.tex <==
% =============================================================================
\section{New linear codes}
\label{sec:new_codes}
% =============================================================================

Hernando et al.~\cite{cota} described a family of codes 
called matrix-product codes with polynomial units
that often render good parameters.
Nevertheless, finding new records is very difficult.
In that work they introduced several new records for small code sizes.

However, for larger code sizes the computation of the minimum distance
took too long with currently available software.
Armed with our new implementations, 
computations that used to take a long time (days or even weeks)
using state-of-the-art software packages can be performed much more quickly.
Taking advantage of this fact, we were able to explore well-known techniques 
to generate new linear codes from this family.

We consider matrix-product codes with polynomial units (see~\cite{hr1})
$ C = [ C_1 C_2 ] \cdot A$, 
where $C_1$ and $C_2$ are cyclic nested codes with the same length $m$ 
and $d_2 > 2 d_1$, 
and matrix $A$ is defined as:
$$
A=
\left(\begin{matrix}
  1 & p \\
  0 & 1
\end{matrix}\right),
$$ where $p$ is a unit in the following ring $\mathbb{F}_2[x]/(x^m -1)$.

We compared the minimum distance of these binary linear codes obtained
with our implementations with the ones in \cite{cota},
the well-known archive of best linear codes.
Later on,
we obtained the following linear codes whose parameters are better than the
ones previously known in \cite{cota}:

\vspace{0.2cm}

%\begin{tabular}{|l|l|}
%\hline From \cite{cota} & New codes   \\ \hline
%$[234,51,62]$ & $\code_1=[234,51,63]$ \\ \hline
%$[234,52,61]$ & $\code_2=[234,52,62]$ \\ \hline
%\end{tabular}

\begin{center}
\begin{tabular}{ll}
\toprule
From \cite{cota} & New codes   \\ \midrule
$[234,51,62]$ & $\code_1=[234,51,63]$ \\ 
$[234,52,61]$ & $\code_2=[234,52,62]$ \\ 
\bottomrule
\end{tabular}
\end{center}

\vspace{0.2cm}

$\code_1=[C_1,C_2] \cdot A$, where $C_1=(f_1)$ and $C_2=(f_2)$ with:

\begin{itemize}

\item $f_1 = x^{67} + x^{59} + x^{54} + x^{51} + x^{49} + x^{42} + x^{39} +
             x^{36} + x^{35} + x^{34} + x^{33} + x^{31} + x^{30} + x^{29} + 
             x^{27} + x^{26} + x^{25} + x^{24} + x^{22} + x^{21} + x^{19} + 
             x^{17} + x^{16 }+ x^{15 }+ x^{14} + x^{13} + x^{11} + x^6 + 
             x^5 + x^3 + x^2 + 1
,$

\item $f_2=(x^{117}-1)/(x+1),$

\item $p = x^{117 }+ x^{116} + x^{115 }+ x^{111} + x^{110} + x^{109} +
           x^{103} + x^{102} + x^{98} + x^{95} + x^{94} + x^{92} + x^{88} + 
           x^{85} + x^{83} + x^{81} + x^{74} + x^{72} + x^{70} + x^{68} + 
           x^{66} + x^{65} + x^{64} + x^{62} + x^{61} + x^{58} + x^{56} + 
           x^{55 }+ x^{54} + x^{51 }+ x^{49} + x^{45} + x^{43} + x^{39} + 
           x^{38} + x^{37} + x^{36} + x^{35} + x^{34} + x^{28} + x^{27} + 
           x^{23} + x^{22} + x^{20} + x^{19} + x^{16} + x^{14} + x^9 + 
           x^7 + x^6 + x^5 + x^4 + x^3 +
x^2 + 1.$

\end{itemize}

$\code_2=[C_1,C_2] \cdot A$, where $C_1=(f_1)$ and $C_2=(f_2)$ with:

\begin{itemize}

\item $f_1 = x^{67} + x^{59} + x^{54} + x^{51} + x^{49} + x^{42} + x^{39} +
             x^{36} + x^{35} + x^{34} + x^{33} + x^{31} + x^{30} + x^{29} + 
             x^{27} + x^{26} + x^{25} + x^{24} + x^{22} + x^{21} + x^{19} + 
             x^{17} + x^{16} + x^{15} + x^{14} + x^{13} + x^{11} + 
             x^6 + x^5 + x^3 + x^2 + 1
,$

\item $f_2 = (x^{117}-1)/(x^2+x+1),$

\item $p = x^{217} + x^{214} + x^{213} + x^{211} + x^{210} + x^{209} +
           x^{207} + x^{205} + x^{203} + x^{202} + x^{200 }+ x^{198} + 
           x^{195} + x^{194} + x^{193} + x^{192} + x^{190} + x^{189} + 
           x^{186} + x^{185} + x^{183} + x^{182} + x^{180} + x^{176} + 
           x^{175} + x^{173} + x^{172} + x^{171} + x^{169} + x^{167} + 
           x^{165} + x^{164} + x^{161 }+ x^{160} + x^{159} + x^{155} + 
           x^{154} + x^{151} + x^{150 }+ x^{148} + x^{147} + x^{144} + 
           x^{143} + x^{142} + x^{141 }+ x^{140} + x^{137} + x^{135} + 
           x^{132} + x^{130} + x^{129} + x^{128} + x^{127} + x^{125} + 
           x^{124} + x^{122} + x^{121 }+ x^{119} + x^{118} + x^{116} + 
           x^{112} + x^{107} + x^{105} + x^{103} + x^{102} + 
           x^{99} + x^{97} + x^{90} + x^{89} + x^{88} + x^{87} + x^{82} + 
           x^{76} + x^{74} + x^{71} + x^{69} + x^{68} + x^{66} + x^{64} + 
           x^{60} + x^{53} + x^{51} + x^{50} + x^{47} + x^{45} + x^{43} + 
           x^{40} + x^{39} + x^{37} + x^{36} + x^{35} + x^{34} + x^{33} + 
           x^{31} + x^{30} + x^{29} + x^{28} + x^{26} + x^{24} + x^{21} + 
           x^{20} + x^{18} + x^{17} + x^{15} + x^{14} + x^{12} + 
           x^8 + x^5 + x^4 + x^3 + 1.$

\end{itemize}

Moreover, operating on $\code_1$ and $\code_2$ we got five more codes:

\vspace{.2 cm}

\begin{center}
\begin{tabular}{cll}
	\toprule
From \cite{cota} & New codes & Method   \\ \midrule
$[235,51,62]$ & $\code_3 =[235,51,64]$ &  Extend~Code ($\code_1$) \\ %\hline
$[236,51,63]$ & $\code_4 =[236,51,64]$ &  Extend~Code ($\code_3$)  \\ %\hline
$[233,51,61]$ & $\code_5 =[233,51,62]$ &  Puncture~Code ($\code_1$,{234}) \\ %\hline
$[232,51,60]$ & $\code_5 =[233,51,61]$ &  Puncture~Code ($\code_1$,{234,233}) \\ %\hline
$[233,52,60]$ & $\code_5 =[233,52,61]$ &  Puncture~Code ($\code_2$,{234}) \\
\bottomrule
\end{tabular}
\end{center}




==> old/crc_tex_toms_rev2/7_Conclusions.tex <==
% =============================================================================
\section{Conclusions}
\label{sec:conclusions}
% =============================================================================

In this paper, we have presented 
several new implementations 
of both the brute-force algorithm and the Brouwer-Zimmermann algorithm
for computing the minimum distance of a random linear code over $\mathbb{F}_2$.
We have compared them with the two most-common implementations 
currently available, \magma{} and \guava{},
in terms of performance, 
obtaining faster implementations in both cases using both sequential 
and parallel implementations, 
each of them either in the scalar or in the vectorized case. 
Finally, we have used our implementation to find out new linear codes 
over $\mathbb{F}_2$ with better parameters than the currently existing ones.
The new ideas and algorithms introduced in this paper 
can also be extended and applied over other finite fields.

Future work in this area will investigate 
the development of specific new algorithms and implementations 
for new architectures 
such as distributed-memory architectures 
and GPGPUs (General-Purpose Graphic Processing Units).


